ContrastMotion: Self-supervised Scene Motion Learning for Large-Scale LiDAR Point Clouds

In this paper, we propose a novel self-supervised motion estimator for LiDAR-based autonomous driving via BEV representation. Different from usually adopted self-supervised strategies for data-level structure consistency, we predict scene motion via feature-level consistency between pillars in consecutive frames, which can eliminate the effect caused by noise points and view-changing point clouds in dynamic scenes. Specifically, we propose \textit{Soft Discriminative Loss} that provides the network with more pseudo-supervised signals to learn discriminative and robust features in a contrastive learning manner. We also propose \textit{Gated Multi-frame Fusion} block that learns valid compensation between point cloud frames automatically to enhance feature extraction. Finally, \textit{pillar association} is proposed to predict pillar correspondence probabilities based on feature distance, and whereby further predicts scene motion. Extensive experiments show the effectiveness and superiority of our \textbf{ContrastMotion} on both scene flow and motion prediction tasks. The code is available soon.

==> sections/abstract.tex <==
% 自动驾驶能够从多种车载传感器例如，相机，激光雷达中受益。最近， there has been a growing interest in 点云学习。

In this paper, we propose a novel self-supervised motion estimator for LiDAR-based autonomous driving via BEV representation. Different from usually adopted self-supervised strategies for data-level structure consistency, we predict scene motion via feature-level consistency between pillars in consecutive frames, which can eliminate the effect caused by noise points and view-changing point clouds in dynamic scenes. Specifically, we propose \textit{Soft Discriminative Loss} that provides the network with more pseudo-supervised signals to learn discriminative and robust features in a contrastive learning manner. We also propose \textit{Gated Multi-frame Fusion} block that learns valid compensation between point cloud frames automatically to enhance feature extraction. Finally, \textit{pillar association} is proposed to predict pillar correspondence probabilities based on feature distance, and whereby further predicts scene motion. Extensive experiments show the effectiveness and superiority of our \textbf{ContrastMotion} on both scene flow and motion prediction tasks. The code is available soon.

%Autonomous driving can benefit from various onboard sensors such as cameras and LiDAR. Recently, there has been a growing interest in point cloud learning. In this paper, we propose ContrastFlow which utilizes abundant unlabeled data for point cloud tasks, including scene flow estimation and motion prediction. Different from previous unsupervised approaches based on structural consistency and regularization, our ContrastFlow is a novel framework based on local feature matching and shows effectiveness and robustness. The encoder learns the discriminative features of different objects or parts of the same object, and then the decoder predicts the flow or motion by feature similarity. Considering rigid motion of objects and sparse point clouds, we also propose \textit{Soft Discriminative Loss} and \textit{Gated Multi-frame Information Fusion Block}. We conduct experiments on KITTI Scene Flow and nuScenes datasets. Our approach performs competitively with other unsupervised methods on KITTI scene flow task and achieves the state-of-the-art result on nuScenes motion prediction task.

% Scene flow involves a pair of 3D point clouds, and predicts which objects in the scene are moving and where they are moving to. Recently, there has been a growing interest in estimating scene flow directly from point clouds. In this paper, we propose ContrastFlow which utilizes abundant unlabeled data for accurate flow estimation. Different from previous unsupervised approaches based on consistency and regularization, we treat the task as a fine-grained classification task. Although the categories are agnostic, our encoder extracts discriminative features of different categories or different objects of the same category. Then a simple query-based decoder estimates scene flow based on feature similarity. Considering rigid motion of objects and sparse point clouds, we also propose Soft Discriminative Loss and Gated Multi-frame Information Fusion Block. In addition, we predict future movements based on historical scene flows. We conduct experiments on KITTI and nuScenes dataset. Our approach performs competitively with other unsupervised methods on KITTI scene flow task and achieves the state-of-the-art result on nuScenes motion prediction task.

% Although the category is agnostic, the encoder treats the corresponding points or voxels in a pair of point clouds as the same category and all points in the same point cloud as different categories. Then a simple query-based decoder gets flow based on category similarity. We also propose some new strategies to satisfy rigid motion and motion smoothing. Experiments on KITTI and nuScenes datasets reveal that our approach performs competitively to other unsupervised methods.

% To this end, we propose a new self-supervised scene flow estimation framework -- ContrastFLow, which is inspired by representing learning and Query Paradigm in 2D, and 3D vision. That is, a simple query-based decoder is enough to get an accurate flow estimation if the encoder can accurately distinguish different aspects of a scene, which trained with the voxel contrast. We conduct our experiences on the FlyingThing3D and KITTI datasets. The results inform the performance of COntrastFlow.

==> sections/conclusion.tex <==
% We demonstrate the results of motion estimation and prediction on KITTI and nuScenes datesets in Figure \ref{fig:RES}. 
In this paper, we propose ContrastMotion, a self-supervised framework in contrastive learning manner for scene motion. We propose Soft Discriminative Loss to bootstrap discriminative feature extraction and alleviate the correspondence missing situations. We also propose Gated Multi-frame Fusion block learning valid compensation
% between point cloud pairs automatically
. 
Pillar association predicts pillar correspondence probabilities 
% based on feature distance, 
and further predicts scene motion.
We will focus on improving the inference speed of pillar association in the future.

==> sections/exp.tex <==

\iffalse
In this section, we first describe the benchmark datasets and experimental setup. Furthermore, we report comparisons to the state-of-the-art methods on the benchmark datasets. Various ablation studies are performed to explain the contribution of each design in our approach. 
\fi

% In the end, we provide the visualization results and analysis.

\subsection{Dateset}
\noindent \textbf{KITTI Scene Flow}~\cite{menze2015joint,menze2018object} consists of 200 training scenes and 200 test scenes. Point clouds and ground truth scene flows are obtained by lifting the annotated disparity maps and optical flows to 3D. Following previous works~\cite{gu2019hplflownet,wu2019pointpwc}, FlyingThings3D (FT3D) dataset, a synthetic dataset with 19640 samples, is used for training and the training scenes in KITTI are used for inference. 

\noindent \textbf{nuScenes}~\cite{nuscenes2019} is a large-scale public dataset for autonomous driving collected from 1000 real scenes, whose initial purpose is object detection and segmentation. The point clouds are captured with a frequency of 20Hz, and  ~\cite{nuscenes2019} annotates the entire dataset with accurate 3D bounding boxes for 23 object classes at 2Hz. Following previous works~\cite{wu2020motionnet,jund2021scalable,li2022rigidflow}, we assume that each object is in rigid motion and derive the ground truth motion from the origin detection and tracking annotations. 

\subsection{Experimental Setup}
\subsubsection{Implementation Details}
We implement all the experiments on PyTorch~\cite{paszke2019pytorch}. For FT3D and nuScenes datasets, we train the ContrastMotion for $300$ and $100$ epochs respectively, and set the initial learning rate to $0.001$, weight decay to $0.001$. The batch size is set to the maximum available on a 32G GPU, and Adam is used as the optimizer. 
% We respectively crop the point clouds in the range $(-35m - 35m)$, and $(0.25, 0.25)$ pillar size.
We crop the point clouds following baseline models~\cite{li2022rigidflow,PillarMotion}, and the pillar size is set to $[0.25, 0.25]$. For training $\mathcal{PC}$ generation, 
% we follow the principles: small rotation, scaling, jitter and large shifts. Specifically, 
the upper limits of shift, rotation angle, scaling and jitter are $3m, 0.17, 1.05$ and $0.1m$. We scale the samples of FT3D to fit the cropping range during training. In KITTI, we predict the motion of points beyond cropping range as the average motion of that scene. The distance threshold $\varepsilon$ in $V(P_i^t)$ is set to $1.1$ times pillar size, and the weights of positive keys $w_{ij}$ are defined as
\begin{equation}
w_{ij} = 
    \begin{cases}
     0.6 & if j = i' \\
     0.1 & else
    \end{cases}
\end{equation}
where pillar $i'$ is the corresponding pillar of pillar $i$. The dimension of output feature map $D=32$.
In pillar association, the patch size $s=32$ and $\alpha=2$. The point clouds from KITTI are more intensive than real scenes. Therefore we adopt a post-processing to scatter the flows of pillars more accurately to points. We randomly select a reference point from each pillar and take the point with the minimum Chamfer~\cite{wu2019pointpwc} loss in corresponding pillar as its corresponding point.
The post-processing mentioned above is not applied to the nuScenes dataset or to the motion prediction task.
In motion prediction task, we predict the motion for the next 1.0s by two past motions for fair comparisons with the methods.
Refer to supplementary materials for more details of the Chamfer Loss and ground points pre-processing.

\subsubsection{Evaluation Metrics}
We report the evaluation criteria used by Hplflownet \cite{gu2019hplflownet} in scene flow: 
\textbf{EPE3D(m)} average end-point-error over each point; 
\textbf{Acc3DS} point ratio where EPE3D $< 0.05$ or relative error $< 5\%$; 
\textbf{Acc3DR} point ratio where EPE3D $< 0.1$ or relative error $< 10\%$;
\textbf{Outliers3D} point ratio where EPE3D $> 0.3$ or relative error $> 10\%$;

\iffalse
\begin{itemize}
    \item EPE3D(m) average end-point-error over each point
    \item Acc3DS point ratio where EPE3D $< 0.05$ or relative error $< 5\%$
    \item Acc3DR point ratio where EPE3D $< 0.1$ or relative error $< 10\%$
    \item Outliers3D point ratio where EPE3D $> 0.3$ or relative error $> 10\%$
\end{itemize}
\fi
We report the average \textbf{L2} distances and \textbf{median} errors on non-empty pillars which are classified as static, slow and fast groups in motion prediction, which used in PillarMotion.

\subsection{Comparison with SOTA methods}
% \yuexin{Maybe rename the following two parts by Scene Flow and Motion Prediction?}
\subsubsection{Scene Flow}
We implement the experiments on FT3D $\rightarrow$ KITTI-SF, and mainly compare our ContrastMotion with the point-based methods, including PointPWC~\cite{wu2019pointpwc}, FlowStep3D~\cite{kittenplon2021flowstep3d}, PoseFlow~\cite{tishchenko2020self} and RCP~\cite{gu2022rcp}, and pillar-based method SLIM~\cite{li2022rigidflow}. Our ContrastMotion and SLIM can process a full scene from KITTI. While the baselines can run inference on a full scene, during training it is infeasible to run them with roughly $30K$ points due to the cost of memory and the training time~\cite{li2022rigidflow}.

% \yuexin{Follow this logic: The performance of point-based methods $\rightarrow$ analyze the reason (their limitations) $\rightarrow$ the performance of pillar-based method, e.g. SLIM $\rightarrow$ its limitation $\rightarrow$ our performance and why we are sota (recall our contributions).}
As shown in Table \ref{tab:KITTT_RESULTS}, the point-based methods, e.g., PointPWC and RCP, achieve limited results compared with the pillar-based approaches. These methods perform significant sampling in the training pipelines due to the heavy cost of memory and computation for large-scale point clouds, while pillar-based methods can be trained with the raw data. The increased points providing more fine-grained information enhance the stable inference ability on the dense point clouds. In Table \ref{tab:KITTT_RESULTS}, we also report the performance of a pillar-based method, SLIM. Although trained with KITTI-RL~\cite{geiger2013vision}, the performance of SLIM is not satisfying, which is due to the effect of point-level correspondence problems in the dynamic scenes. Our ContrastMotion leverages feature-level consistency to predict pillar flows and achieves SOTA performances in EPE3D and Outliers3D metrics. The results show the effectiveness of pillar-based methods and our ContrastMotion. 
% Furthermore, Compared with point-level correspondence, matching correspondences using the high-level feature reduce the effect of correspondence problems and works well in scene flow tasks.

% \textcolor{red}{ Our ContrastMotion achieves the SOTA performances in EPE3D and Outliers3D metrics and comparable performances in other metrics. From the performances of ours and SLIM, We believe that increased point cloud density provides more fine-grained information and represents a domain shift for the networks during inference, which also mentioned in SLIM. Compared to most point-based motion estimation approaches trained on down-sampled point clouds, our ContrastMotion can work with the raw data which has more fine-grained information compared to the down-sampled data and facilitates pillar matching based on feature similarity and point matching based on structural information.}
In order to get closer to real-world evaluation, we also implement self-supervised experiments on the dataset without point correspondences, nuScenes, and compare our ContrastMotion with SLIM~\cite{li2022rigidflow}. As shown in Table~\ref{tab:nuScene_flow}, Our ContrastMotion achieves the SOTA performance in moving EPE3D. Where around 95\% points in nuScenes are static. Our proposed GMF enhances the feature consistency between the corresponding static pillars and helps our ContrastMotion achieve the best performance compared to the baseline methods in static EPE3D.


\subsubsection{Motion Prediction}
As same as PillarMotion~\cite{PillarMotion}, we use the same 500 training scenes, 100 validation scenes and 250 testing scenes with PillarMotion \cite{PillarMotion} .But unlike PillarMotion which uses LiDAR, camera and pose data, only LiDAR and pose data are used in our work.
The related methods we compare include self-supervised PillarMotion~\cite{PillarMotion}, and pre-trained supervised estimators on other datasets, e.g., FlowNet3D~\cite{liu2019flownet3d} and HPLFlowNet~\cite{gu2019hplflownet}. 
% In addition, we report the performance of the static model assuming the environment is static.

Table~\ref{tab:NUSCENES_RESULTS} shows the results of different approaches. The performances of FlowNet3D and HPLFlowNet which are trained in FT3D and tested on nuScenes without fine-tuning indicate the existence of a large domain gap. In addition, 3D labeling on real large-scale scenes requires complex processes and labor-intensive human efforts, and the discrepancy is obvious for cross-scenes and cross-LiDAR captured data. PillarMotion achieves a limited performance with consistency and cross-device regularization, which is also due to the effect of point-level correspondence missing in the dynamic scenes. In addition, the optical flow used as a signal to guide motion learning introduces errors, including optical flow prediction and coordinate transformation errors. Our ContrastMotion achieves SOTA performances among the compared methods in the low and high speed groups, and the prediction errors decrease by $35\%$ and $0.02$ compared to PillarMotion. In terms of median errors, our ContrastMotion achieves SOTA performances in all the groups. The results show the advantages of self-supervision compared with supervision and the potential of ContrastMotion in motion prediction tasks.



\subsection{Ablation Studies}
% We perform experiments to explore the effects of proposed GMF, Ground Mask and SD--Loss on performances.
% \begin{table*}[t]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%     \hline
%         \multicolumn{2}{|c}{Loss} & \multicolumn{2}{|c}{Ground} & \multicolumn{2}{|c}{Gated. Block} & \multirow{2}*{Stcatic} &  \multirow{2}*{Speed $\le$ 5m/s} &  \multirow{2}*{Speed $>$ 5m/s}\\
%         Soft. (ours) & PointInfoNCE & w/ & w/o & w/ & w/o \\
%         \hline
%         \checkmark & & & \checkmark & \checkmark & & 0.2687 & \textbf{0.4952} & \textbf{2.2581} \\
%          & \checkmark & & \checkmark & \checkmark & & 0.2697 & 0.6546 & 2.9601 \\
%          \checkmark & & \checkmark & & \checkmark & & \textbf{0.1982} & 0.4979 & 2.9872 \\
%          \checkmark & & \checkmark & &  &\checkmark & 0.4777 & 0.7791 & 2.9497 \\
%     \hline
%     \end{tabular}
%     \caption{Comparison of our models using different combinations of the soft discriminative loss, ground removal, and gated multi-frame information fusion block. We evaluate each model on nuScenes scene flow task and report mean errors.}
%     \label{tab:ABL}
% \end{table*}


\subsubsection{Gated Multi-frame Fusion Block}
% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|c|c}
%     \hline
%         Method & \multicolumn{2}{|c}{ContrastFlow} \\
%         \hline
%         Block & w/ &  w/o \\
%         \hline
%         Static & 0.0.1982 & 0.4777 \\
%         Speed $\le$ 5m/s & 0.0.4979 & 0.7791 \\
%         Speed > 5m/s & 2.9872 & 2.9497 \\
%     \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:W_WO_BLOCK}
% \end{table}

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\columnwidth]{HEAT.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{\textbf{The pillar description maps $\mathbf{m}$ generated by Gated Network in \textit{GMF}.} The red boxes indicate moving objects. Overlaying the description maps on the point clouds, we can see that there are $m$ close to \textit{zero} in positions where movable objects and empty pillars appear, but there are $m$ close to \textit{one} in positions where static objects such as ground, road edges, etc., appear.}
\label{fig:HEAT}
%\vspace{-2ex}
\end{figure}


% \yuexin{Redundant here. Describe the experiment, give analysis on performance, and finally stress the effectiveness.}\textcolor{blue}{The corresponding points cannot be accurately re-scanned at the next timestamp due to \yuexin{ego-motion?} ego-motion and occlusion, which is adverse to the pillar and point association. However, consecutive frames provide much more perspectives on the same scene, and the fusion of information from different perspectives enables a better understanding of the scene, especially for backgrounds and static objects. Considering that direct fusion of multiple frames will introduce extra noises, we design a gated multi-frame fusion block (GMFB) to achieve feature fusion between consecutive frames.} 
We perform experiments to explore the effects of proposed GMF, and the results are shown in Table \ref{tab:ABL}. The baseline model (a) trained only with our SD--Loss does not perform well for static and low speed group. However, model (b) incorporating of proposed GMF performs significantly better in the static and low speed groups, and achieves comparable performances with (a) in high speed group. 
% which shows that the GMF learns the valid compensation and further benefit the accuracy of static and low-speed object motion estimation. 
In addition, we visualize the pillar description maps in GMF, which represents the probability of inserting the features of each pillar to another point cloud feature map. As shown in Figure~\ref{fig:HEAT}, there are significantly high mask values in positions without motions, such as the ground, but low values where movable objects and empty pillars appear. What is mentioned above shows GMF learns valid movable-static information and compensation, and further enhance the feature consistency between corresponding pillars which facilitates the pillar association to acquire accurate pillar correspondence.
% \yuexin{Have you compared with the direct warping as mentioned in Method.5?}



\iffalse
\subsubsection{Ground Mask} 
% \yuexin{Move it after SD-Loss since it is not our novelties. Use simple words here.} The ground is the static background for point cloud tasks. Compared with the supervised learning approaches which implicitly distinguish between foreground and background, neither the scene consistency nor feature matching based unsupervised approaches can avoid the failing estimations of the ground points. For examples, the related works~\cite{wu2019pointpwc, gu2022rcp, li2022rigidflow} set the threshold value to ignore the ground points in KITTI Scene Flow dataset. When generating the point cloud $\mathcal{P}_t+1$ during the contrast training, we apply the transformation to all the points of $\mathcal{P}_t$ which results in the same displacements of the background and foreground and leverage the unsupervised JCP ground segmentation algorithm to remove the ground points in pre-processing to correct the motions of the ground. 
We conduct experiments (b) and (c) regarding whether to feed the ground points to ContrastMotion, and the results are shown in Table~\ref{tab:ABL}. Although the ground is processed differently, the evaluations are performed on the original point clouds in nuScenes. Model (b) achieves the leading performance in the static group, but model (c) performs better in the movable groups. We believe that model (b) learns the features of the ground and distinguishes the background. However, the presence of the ground points affects the discriminative features of the movable objects due to the sparse point cloud and pillar representation, which degrades its performance on movable groups. Although the false negative ground points affect the performance of model (c) in the static group, it has better overall performance.
\fi

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\columnwidth]{HS.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{ \textbf{The corresponding probabilities between points in $T+1$ and the reference points in $T$ inferred from model (c) and model (d), which respectively adopt SD--Loss and PointInfoNCE as loss function.} Top row: a false negative estimation by model(d). Middle row: a false positive estimation by model (d). Bottom row: the case that the corresponding points are not scanned. For all cases, model (c) which adopt proposed SD--Loss provides reasonable results.}
\label{fig:HS}
\end{figure}

\subsubsection{Soft Discriminative Loss}
We also conduct experiments to compare proposed SD--Loss with PointInfoNCE proposed by PointContrast~\cite{xie2020pointcontrast}. Comparing models (c) and (d) in Table \ref{tab:ABL}, we find that model (c) achieves better performances in all the groups. As shown in Figure~\ref{fig:HS}, we believe that SD--Loss considering the feature similarities of the local points can make an approximate estimation in the case that the corresponding points are not scanned and the corresponding probabilities inferred by model (c) show a Gaussian-like distribution due to the soft pillar correspondence adopted in SD--Loss, which provide a margin of fault tolerance and avoid the destruction of noises and changing views of dynamic scenes.

\iffalse
Figure \ref{fig:HS} shows the corresponding probabilities of $P_j^{t+1}$ with reference $P_i^t$. As expected, models (c) and (d) push the pillars away from each other and scatter them in the feature space. However, model (d) trained with PointInfoNCE makes false negative estimations as shown in the top row, and the corresponding probabilities inferred by model (c) show a Gaussian-like distribution due to the soft pillar correspondence adopted in SD--Loss. In the middle row, the points having high corresponding probabilities estimated by model (d) are not the corresponding points of the reference; that is model (d) makes a false positive estimation. The estimations of (d) are destroyed in the case that the corresponding points are not scanned, as shown in the bottom row. However, model (c) considering the feature similarities of the local points makes an approximate estimation. The results show that proposed SD--Loss provides a margin of fault tolerance and avoids the destruction of noises and changing views of dynamic scenes.
\fi

For 
% visualization of inference results of model (c) and (d), 
ablation experiments of ground points, qualitative and runtime analysis, please refer to the supplementary material.
% \yuexin{Have you done ablation for your key number?}

==> sections/introduction.tex <==
For autonomous vehicles, it is critical to understand the dynamic cues in large-scale scenarios, e.g. distinguishing movable and static objects in the environment, to avoid obstacles and guarantee the safety~\cite{mahjourian2018unsupervised,luo2018fast}. Due to the advantage of long-range depth capture, LiDAR has become one popular sensor for scene perception~\cite{Cong_2022_CVPR,Yin2020Centerbased3O,Zhu2020SSNSS,zhu2021cylindrical} and boosted the development of autonomous driving. Extracting motion features from LiDAR point cloud has attracted more and more attention in recent years, which is a fundamental technique for many downstream tasks, such as detection, segmentation, trajectory prediction, navigation, etc. 

\begin{figure}[htb]
\centering
\includegraphics[width=1.0\columnwidth]{fig1.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{ \textbf{The corresponding probabilities between pillars in $T+1$ and the reference pillar (red cross) in $T$ inferred from ContrastMotion.} ContrastMotion extracts discriminative features based on geometric context information and predict corresponding probabilities between pillars in $T+1$ and the reference based on feature distance. The transition from red to green indicates that the corresponding probability is decreasing.}
\label{fig:segmatation}
\end{figure}

However, 3D labeling on large-scale point clouds requires complex processes and labor-intensive human efforts. Unlike the regular pixel representation of images, LiDAR point cloud is sparsity-varying and unordered in one scene and the discrepancy is more obvious for cross-scenes and cross-LiDAR captured data, leading to the situation that supervised methods are difficult to adapt to other domains. Considering above limitations, we focus on the self-supervised learning strategy to extract the motion pattern existing in consecutive frames of LiDAR point cloud.


%For surveillance and autonomous vehicles (AVs), it is critical to understand the dynamic cues in large scale scenarios. In AVs, scene flow distinguishes between movable and static objects in the environment \cite{casas2018intentnet} and helps in downstream tasks such as tracking and obstacle avoidance \cite{mahjourian2018unsupervised, luo2018fast}, which enables AVs to navigate in a complex environment. Further, scene flow is a set of vectors of 3D displacements between corresponding elements in two consecutive frames, which provides information about the motion of the current scene and can be used to predict future motion.

Scene motion is a fine-grained representation of the motion pattern, which is defined as a 3D displacement vector between each point in two sequential frames~\cite{wu2019pointpwc}. There are already some self-supervised approaches~\cite{gu2022rcp,baur2021slim,li2022rigidflow} for scene flow estimation. However, most of them rely on point-wise feature extraction and correlation corresponding, which bring heavy costs of memory and computation for large-scale point clouds. Meanwhile, the data-level structure consistency is not applicable for dynamic scenes, because LiDAR is view-dependent and will capture different views of objects in different frames, causing many points having no correspondences in adjacent frames and leading to low accuracy for the motion estimation. These properties limit the deployment of such methods in real scenes, which is highly dynamic and requires high-efficiency point cloud processing.


%Recently, LiDAR has become one of the most commonly used sensors on self-driving vehicles, and the approaches of learning directly from point clouds have received a lot of attention. The related works \cite{} have shown the advantages and potential of point clouds for various perceptual tasks. However, 3D labeling requires complex pipelines and labor-intensive human effort. The lack of labels discourages the evolution of the point cloud tasks. Unlike supervised learning which requires laborious labeling, unsupervised learning opens up the possibility to utilize a practically infinite train data size, and has grown significantly along with the explosive growth of low-cost data. In especially, training from a unsupervised pre-trained model has become the dominant approach in some fields.

% The unsupervised approaches \cite{} based on point cloud consistency have achieved excellent performance in scene flow and motion prediction tasks, and we propose a novel unsupervised framework for point cloud learning. The point cloud consistency approaches estimate optimal global matching, while our ContrastFlow estimates precise local matching of the essential elements of the point cloud. With more attention to local geometric information, our ContrastFlow is more sensitive to fine-grained discriminative features, so it has strong robustness and transferability on fine-grained tasks.

% Because the point cloud is a sparse representation of the object, the reference points of the object cannot correspond one by one in two frames, and the ground truth flow is ambiguous. Therefore, some approaches use synthetic data in the training process, e.g. FlyThings3D dataset. However, models trained with synthetic data show limited performance due to the domain gap between synthetic and real scene. Others use other types of labels to generate ground truth scene flow, such as detection labels.  


Instead of dense motion prediction, researchers tend to explore the motion representation on Bird's Eye View (BEV). Due to the rich semantic and geometry information existing in the BEV representation, especially for the traffic scenarios, BEV provides a trade-off choice for accurate and efficient perception in large-scale scenes~\cite{ma2022vision}. Moreover, BEV representation can, to some extent, eliminate the effect caused by unordered and noisy points by discretizing the point cloud into BEV grid cells. Such compact representation is friendly for defining the search window for point matching. Thus, based on one popular BEV~\cite{li2022bevformer} and pillar~\cite{lang2019pointpillars} representation, , ~\cite{PillarMotion,baur2021slim} propose effective motion estimators, which are more applicable for autonomous driving. However, the self-supervised architecture is similar to previous scene flow methods by mainly using the point-level structure consistency and regularization between consecutive frames of point cloud for self-supervision. Such methods, depending on data-level correspondences, still suffers from dynamic changes of scenes.

%Recently, the unsupervised approaches \cite{wu2019pointpwc, PillarMotion} based on structural consistency have achieved excellent performance in scene flow and motion prediction tasks. Apparently, the structural consistency relies on the existence of corresponding points between two consecutive point clouds. However, the corresponding points cannot be re-scanned exactly at the next timestamp, and they can be obscured or get out of sensor range \cite{PillarMotion}. In addition, PointPWC \cite{wu2019pointpwc} introduces a novel cost volume via inner product. The cost quantity is the similarity between the features at each point and serves as auxiliary information for estimating the scene flow. PointPWC demonstrates the potential of feature similarity in solving scene flow estimation tasks. Therefore, we propose, ContrastFlow, a novel unsupervised framework based on feature similarity. Based on bird's eye view (BEV) representation, our ContrastFlow uses pillars as the essential matching elements. Considering that the point cloud is sparse and the point correspondence is ambiguous, the pillar-based matching reduces the dependence on point correspondence and maintains accurate correspondence after down-sampling. BEV representation can handle large-scale scenes with a stable resource footprint and facilitate multi-sensor information fusion, deployment. Futher, BEV representation and pillar-based models have become the main approaches in AVs. Compared with structural consistency based regression approaches, our ContrastFlow estimates flow by feature matching. ContrastFlow extracts the discriminative features of different pillars and then associates the corresponding pillars based on feature similarity. As shown in Figure \ref{fig:segmatation}, for each reference pillar, ContrastFlow extracts discriminative features based on its surrounding geometric information, and then locates the pillar with the most similar features to the reference in the next frame. The feature similarity shows a Gaussian distribution due to the similarity of local geometric information. In addition, ContrastFlow still gives accurate matches even for similarly shaped objects, which illustrates the effectiveness of ContrastFlow for discriminative feature extraction.


In this paper, based on the pillar representation, we propose a novel self-supervised scene motion estimator for LiDAR captured large-scale point clouds, which has solved above problems. To reduce the effect of point-level correspondences missing during the view-dependent scanning in dynamic scenes, we extract the high-level feature representation of each pillar and then predict pillar corresponding probabilities between consecutive frames (Fig \ref{fig:segmatation}). After obtaining the pillar correspondences, we easily calculate the motion information of the whole scene. Specifically, we utilize contrastive learning to bootstrap the network to extract discriminative features of each pillar, where the
% by pulling pillar features belonging to positive pillar pairs closer and pushing features of negative pairs away.
positive pillar pairs are two pillars that have a corresponding relationship in consecutive frames. To acquire positive pairs without any labels, we leverage commonly used data augmentation methods to generate two frames of point clouds from the same sample and record the pillar correspondences according to the transformation matrix. Although the hard one-to-one positive pillar assignment increases the discriminability of features, it provides less supervision and makes it difficult for the network to learn strong and robust features. Therefore, we propose \textit{Soft Discriminative Loss(SD--Loss)}, which generates positive pillar pairs with a soft constraint to further provide a margin of fault tolerance in the dynamic scenes. We also propose \textit{Gated Multi-frame Fusion (GMF)} block learning valid compensation to enhance feature consistency of corresponding pillars, where the gate status also provides dynamic and static information about the scene. In \textit{pillar association}, we predict the pillar correspondence probabilities mainly through the feature distance of pillars between consecutive frames. Moreover, in order to reduce the complexity of pillar association from quadratic of the number of pillars to linear, we adopt \textit{Patching} and \textit{Asymmetric Patch} strategy.

%There are still some challenges in feature similarity calculation and matching: (1) how to extract discriminative features of the pillars; and (2) the high computational complexity in large-scale autonomous driving scenes. For discriminative feature extraction, we train the encoder of ContrastFlow with contrast learning. Contrast learning pulls pillar features in positive pairs closer and pushes them in negative pairs apart, where corresponding pillars are considered as positive pairs and non-corresponding pillars as negative pairs. Considering the similarity of the neighboring pillars, ContrastFlow calculates the loss using the soft correspondence approach, i.e. Soft Discriminative Loss. We feed the point cloud pairs into the shared encoder, obtain the feature maps, and then calculate the feature similarity of different pillar pairs. However, the complexity of calculating the similarity between all pairs is $O(n^2)$. Therefore, for each pillar in the first frame, we set a window of $S*S$ in the next frame and calculate the similarity to the pillars within the window only. By using the query window, we reduce the computational complexity to linear. 


%The related point cloud works \cite{vora2020pointpainting, wu2020motionnet, PillarMotion} warp the multi-frame point clouds to enhance the objects feature extraction, considering the occlusion and object loss when the viewpoint changes. Therefore, we propose Gated Multi-frame Information Fusion Block, which aggregate information of point cloud pairs directly on the feature maps. The block predicts the gating values from the feature maps, which control the message passing between point clouds. Therefore, we propose Gated Multi-frame Information Fusion Block, which aggregate information of point cloud pairs directly on the feature map. The block predicts the gating value from the feature map, which controls the message passing between point clouds.

% Considering occlusion and objects loss as the viewpoint changes, the related point cloud works  distorts the multi-frame point clouds to enhance the feature extraction of the objects. 
% Although there are works \cite{baur2021slim, li2021neural, pontes2020scene} related to scene flow on the nuScenes dataset, these works do not specify how to split the training and test sets and we cannot make a fair comparison with them.

We validate our ContrastMotion on the KITTI Scene Flow dataset and nuScenes dataset and achieve state-of-the-art performance for both scene flow and motion prediction tasks. We also conduct ablation studies to illustrate the effectiveness of the novel designs in our method.

The contributions of our work can be summarized as follows.
\begin{itemize}
\item We propose a novel pillar-based self-supervised motion estimator for LiDAR point cloud, which predicts pillar corresponding probabilities between point cloud pair by feature distance, and further acquires scene motion.

\item We propose Soft Discriminative Loss(SD--Loss) to provide the network with more pseudo-supervised signals to learn discriminative and robust features, and it can also tackle the case of correspondence points missing in real scenes.

\item We propose Gated Multi-frame Fusion(GMF) block learning valid compensation between point cloud pairs automatically to enhance feature consistency of corresponding pillars, which also has the capability of perceiving dynamic-static information of the scene.

\item We analyze the degradation solution, and our ContrastMotion has achieved state-of-the-art performance on both scene flow estimation and motion prediction tasks.
\end{itemize}



\begin{figure*}[htb]
\centering
\includegraphics[width=1.8\columnwidth]{MODEL} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \caption{A schematic overview of the proposed self-supervised motion estimator for LiDAR point cloud. We introduce a feature-level consistency augmented with \textit{SD--Loss} to achieve self-supervision in a contrastive learning manner. We also propose \textit{Gated Multi-frame Fusion} block learning valid compensation to enhance feature similarity of corresponding pillars}
\label{fig:ContrastFlow}
\end{figure*}

==> sections/method.tex <==
% \yuexin{Follow this organization: 1.Preliminaries, 2.Overview (The whole pipeline according to Fig.2 and stress important modules.), 3.Contrast Learning (3.1.Self-contrast and Cross-contrast, 3.2.Soft Discriminative Loss), 4.Pillar Association, 5.Gated Multi-frame Fusion Block, 6. Task-specific Post-processing (6.1 Scene Flow, 6.2 Motion Prediction). \\\\ For the section of 3-6, give the motivation first, then describe how you do, and finally point why your operation can solve the concern in the motivation.}

\iffalse
\subsection{Preliminaries}

We represent the point cloud at time $t$ as $\mathcal{PC}_t = {\{p_i^t\}}_{i=1}^{Nt}$, where $p_i^t$ represents one point and $N_t$ represents the number of points. 
BEV provides a trade-off choice for accurate and efficient perception\cite{lang2019pointpillars,li2022bevformer,park2021pseudo,wang2022detr3d} by discretizing point clouds into grid cells. 
Considering the efficiency requirement in dealing with large-scale point cloud for autonomous driving, the encoder of our ContrastMotion is based on the popular BEV representation, pillars, rather than points. The point cloud $\mathcal{PC}_t$ are discretized into pillars $\{P_i^t\}_{i=1}^{N_p}$, where $N_p$ is the number of pillars.
\fi

% \yuexin{Delete and merge this part with the related work with simplified description.}\textcolor{blue}{ContrastMotion discriminates features in a contrast learning manner. Contrast Learning has attracted more and more attention in unsupervised domains recently, which pulls the cells of positive pairs closer and pushes the cells of negative pairs apart in the feature space. In 3D computer vision, PointContrast \cite{xie2020pointcontrast} relates the corresponding points in different views, while ContrastMotion makes connections between consecutive frames of the point clouds. ContrastMotion is inspired by PointContrast, but still different:}
% \begin{itemize}
%     \item \textcolor{blue}{PointContrast, a pre-training approach, aims at feature representation learning, while ContrastMotion aims at solving the motion estimation task by feature matching;}
    
%     \item \item \textcolor{blue}{PointContrast is a point-based model, while ContrastMotion is based on pillars representation considering the large-scale scene of autonomous driving;}
    
%     \item \item \textcolor{blue}{We propose soft discriminative loss to match similar features with a soft constrain due to the fact that the correspondence of points in consecutive frames is ambiguous.}
% \end{itemize}

\subsection{Overview}
We represent the point cloud at time $t$ as $\mathcal{PC}_t = {\{p_i^t\}}_{i=1}^{Nt}$, where $p_i^t$ represents one point and $N_t$ represents the number of points. 
% BEV provides a trade-off choice for accurate and efficient perception\cite{lang2019pointpillars,li2022bevformer,park2021pseudo,wang2022detr3d} by discretizing point clouds into grid cells. 
Considering the efficiency requirement in dealing with large-scale point cloud for autonomous driving, the encoder of our ContrastMotion is based on the popular pillar representation. The point cloud $\mathcal{PC}_t$ are discretized into pillars $\{P_i^t\}_{i=1}^{N_p}$, where $N_p$ is the number of pillars.

% \yuexin{Add a new subsection after Preliminaries in the method section, called 'Overview'. And move the following text to it. Just use conclusion words in the caption. For the text in the figure, please use 'Times New Roman' style.}
As shown in Figure \ref{fig:ContrastFlow}, our ContrastMotion is in a contrastive learning mechanism. 
%ContrastMotion consists of contrastive training and pillar association. The training pipeline of ContrastMotion contains self-contrast and cross-contrast in a contrastive learning manner and is supervised by proposed soft discriminative loss. Self-contrast learns the discriminative features of different pillars in the same frame; Cross-contrast learns the similar features of corresponding pillars in consecutive frames. 
In training pipeline, We leverage commonly used data augmentation methods to generate $\mathcal{PC}_t$ and $\mathcal{PC}_{t+1}$ from the same point cloud sample, learn the representations of $\mathcal{PC}_t, \mathcal{PC}_{t+1}$ organized in pillars with \textit{PFE}~\cite{qi2017pointnet}, and then feed them to our \textit{Encoder} which is similar to backbone in FastFlow3D~\cite{jund2021scalable}, respectively. After that, The Gated Multi-frame Fusion(GMF) block learn valid compensation to enhance feature consistency of corresponding pillars, and its outputs are two flattened feature maps of $N_p \times D$, where $N_p$ is the number of pillars and $D$ denotes feature dimension. We then predict pillar corresponding probabilities based on feature distance between pillars in point cloud pair.
The errors between predicted pillar corresponding probabilities and ground truth pillar correspondences are taken as the loss to optimize parameters. Given consecutive frames during inference, ContrastMotion 
generates pillar correspondences based on pillar corresponding probabilities, and further scene motion. 
% The process is named pillar association, where we adopt \textit{Patching} and \textit{Asymmetric Matching} strategy considering efficiency and accuracy. %The post-processing associates points within the pillar pairs via structural information if there is a point motion task. 
% Finally, we will provide post-processing for specific motion tasks, including scene flow estimation and motion prediction.

% \yuexin{Merge into the 'Overview' subsection.}\textcolor{blue}{  In pillar association pipeline, we calculate the feature similarity between pillars and then take the displacements between the pillars with the greatest similarity as the motions. In addition, we design a gated multi-frame fusion block to learn the valid compensation from consecutive frames.}
% \yuexin{Introduce the pillar processing and encoder in the 'Overview' subsection.}\textcolor{blue}{Different from the approaches supervised by data-level correspondences and structural consistences which suffer from dynamic changes of scenes, self and cross contrast learn the motion information via feature-level correspondences. Based on BEV representation, ContrastMotion discretize points into non-overlapping pillars and feed them to the shared encoder~\cite{jund2021scalable} which performs twice down sampling and up sampling. The roles of the shared encoder are (1) to aggregate contextual geometric information and (2) to project the pillars to an easily discriminable higher dimensional feature space. }


\subsection{Contrastive Learning}

\subsubsection{Self-contrast and Cross-contrast}
Different from the methods with point-level correspondences and structural consistency suffering from dynamic changes of scenes, we learn the motion pattern via feature-level consistency. To learn the discriminative features distinguishing each pillar from others and feature consistency between corresponding pillars, we formulate the problem as a one-to-$N_p$ classification task in contrastive learning, and propose \textit{Self-contrast} and \textit{Cross-contrast}

Specifically, Self-contrast and Cross-contrast are used for learning the discriminative features of different pillars in the same frame and feature consistency of corresponding pillars in consecutive frames, respectively. For the former, each pillar forms a positive pair with itself only and forms the negative pairs with all others in the same frame. For the latter,
since there are no pillar correspondence labels for consecutive frames in self-supervised training, we leverage commonly used data augmentation methods to generate $\mathcal{PC}_{t}$ and $\mathcal{PC}_{t+1}$ from the same point cloud training sample, including random rotation, shift, scaling, and jitter. All the data augmentation transformations are applied to the entire point clouds to ensure the completeness of the object surfaces. Then we acquire pillar correspondences based on the known transformation matrices in data augmentation, where each pillar ${P}_i^t$ forms a positive pair with its corresponding pillar ${P}_{i'}^{t+1}$ and negative pairs with all other pillars ${P}_{j}^{t+1}$ where $j \neq {i'}$. After that, the feature consistency of corresponding pillars can be learnt by Cross-contrast in a contrastive learning manner. In addition, we apply the random removal to the points in generated $\mathcal{PC}$ to simulate the change in the appearance of the objects caused by ego-motion to avoid over-fitting. Self-contrast and Cross-contrast learn the discriminative and consistent pillar features on which pillar corresponding probabilities depend, which reduces the effect of noise points and point correspondences missing in dynamic scenes.

\subsubsection{Soft Discriminative Loss}
As mentioned above, The training pipeline of Self- and Cross-contrast is considered a contrastive learning manner. For unsupervised contrastive learning, InfoNCE~\cite{oord2018representation} and PointInfoNCE proposed by PointContrast~\cite{xie2020pointcontrast} are widely used recently. Specifically, they encourage one query to be similar to one positive key and dissimilar to, typically many, negative keys. However, the one-to-one correspondence is not applicable for dynamic scenes, because LiDAR is view-dependent and will capture different views of objects in different frames, causing many points having no correspondences in adjacent frames. Moreover, most points of one rigid object have similar motion and contextual geometric information. Therefore, we generate positive keys with a soft constraint and propose soft discriminative loss (SD-Loss).

\begin{equation}
    \mathcal{L} = -\sum_{i}\sum _{j\in V(P_i^t)} w_{ij} log \frac{exp(\sigma (P_i^t) * \sigma (P_j^{t+1}) )}{\sum _{k}exp(\sigma (P_i^t) * \sigma (P_k^{t+1}))} 
\end{equation}
Here $*$ denotes vector inner product. $V(P_i^t) = \{P_j^{t+1} | d(P_j^{t+1}, P_{i'}^{t+1}) < \varepsilon \}$ represents the positive keys of $P_i^t$, where $d(\cdot, \cdot)$ is the Euclidean distance function, $ P_{i'}^{t+1}$ is determined by the transformation matrix and the corresponding pillar of $P_i^t$, and $\varepsilon$ represents the distance threshold. $\sigma (x)$ is the pillar features extracted by the networks, where $ReLU$ guarantees a positive feature vector, and $w_{ij}$ represents the weight of each positive key, which has a negative correlation with the distance between pillar $P_j^{t+1}$ and $P_{i'}^{t+1}$. For each pillar $P_i^t$, we generates the weighted positive keys with not only the corresponding pillar $P_{i'}^{t+1}$ defined by transformation matrix but also the neighbouring pillars of $P_{i'}^{t+1}$. Compared to the PointInfoNCE, our SD--Loss retains the feature similarities of local pillars and provides a margin of fault tolerance to avoid the destruction of changing views of point clouds in dynamic scene. Moreover, SD--Loss tackles a widely observed challenge that one-to-one positive key assignment provides less supervision, making it difficult for the network to learn strong and robust features.

\iffalse
\subsection{Ground Removal}
Not only for motion task but for registration~\cite{Li_2021_CVPR,Bai_2021_CVPR,DBLP:conf/aaai/ChenYT22,DBLP:conf/aaai/XuYLZL22} and odometry~\cite{wang2021pwclo}, the ground is a special \textit{stuff}. The ground points are continuous and are not captured at the same location due to ego-motion between adjacent frames. Furthermore, the ground points have the same texture and weak discriminative features. Therefore, most methods suffer from the ground points and remove the ground in pre-processing to avoid their destroy. In KITTI Scene Flow dataset, we remove the ground points below a threshold height following PointPWC~\cite{wu2019pointpwc}. We remove the ground points in nuScenes samples with the unsupervised ground segmentation algorithm based on Jump-Convolution-Process (JCP)~\cite{shen2021fast}.The algorithm leverages the gradient of the point, ring index and other information to segment the point cloud, and then reclassifies the images mapped from the point cloud with JCP. The motions of the ground points can be set to zero easily.The ground removal avoid the destruction of the ground for foreground object features, which is not explicitly mentioned by the related works~\cite{PillarMotion} in nuScenes.
\fi


% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c}
%     \hline
%      Points & Method & EPE3D(m)$\downarrow$ & Acc3DS$\uparrow$ & Acc3DR$\uparrow$ & Outliers3D$\downarrow$ \\
%     \hline
%     % \multirow{5}*{8192} & ICP(rigid) \cite{besl1992method} & 0.5181 & 0.0669 & 0.1667 & 0.8712 \\
%     % ~ & FGR(rigid) \cite{zhou2016fast} & 0.4835 & 0.1331 & 0.2851 & 0.7761 \\
%     % ~ & CPD(non-rigid) \cite{myronenko2010point}& 0.4144 & 0.2058 & 0.4001 & 0.7146 \\
%     \multirow{5}*{All} & PointPWC \cite{wu2019pointpwc} & 0.3648 & 0.0726 & 0.2974 & 0.8579 \\
%     ~ & PoseFlowNet~\cite{tishchenko2020self} & 0.3256 & 0.1104 & 0.2058 & 0.9778 \\
%     ~ & RCP~\cite{gu2022rcp} & 0.0974 & 0.6058 & 0.8021 & 0.3263 \\
%     ~ & FlowStep3D~\cite{kittenplon2021flowstep3d} & 0.2298 & 0.4593 & 0.6324 & 0.4886 \\
%     ~ & RobOT~\cite{shen2021accurate} & - & - & - & - \\
%     ~ & ContrastMotion (ours) & \textbf{0.0815} & 0.7321 & 0.83615 & \textbf{0.2081} \\
%     \hline
%     \end{tabular}
%     \caption{\textbf{Evaluation results on FT3D -$>$ KITTI Scene Flow.} All the methods are self-supervised trained only on FT3D and evaluated on KITTI Scene Flow dataset. PointPWC, FlowStep3D, RobOT, RigidFlow and RCP are point-based model, while ours and SLIM are pillar-based. *: models trained on KITTI~\cite{geiger2013vision}.}
%     \label{tab:KITTT_RESLTS}
% \end{table*}

\subsection{Gated Multi-frame Fusion Block}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\columnwidth]{Gated.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
% \caption{After training our ContrastFlow, we calculate the feature similarity of the points in the search space to the reference points in the first frame. The first row shows the feature similarity of different parts of the same object, and the second row shows some other objects.}.
% \label{fig:segmatation}
% \end{figure}
 
% The related works~\cite{vora2020pointpainting, wu2020motionnet, PillarMotion} warp the multi-frame point clouds to enhance the objects feature extraction, considering the occlusion and object loss when the viewpoint changes.
Adjacent frames can provide additional information to enhance the features of current sparse point cloud. However, naive fusion of multiple frames makes the moving objects trailing and makes the pillar association which relies heavily on the feature consistency of pillars ambiguous. Therefore, we propose Gated Multi-frame Fusion(GMF) block to learn the valid complement features from adjacent frames, which consists of a gated network. After the \textit{Encoder} extract the features $\mathbf{F}_t$ and $\mathbf{F}_{t+1}$, we align two feature maps according to ego-motion to make the features at the same grid correspond to the same real-world location.
Considering a static scene, the fusion feature can be denoted as $\mathbf{F}_t + \mathbf{F}_{t+1}$ due to warping ego-motion between consecutive frames.
To avoid wrong fusion caused by moving objects in real scene, we introduce pillar description maps.
We feed $\mathbf{F}_t$ and $\mathbf{F}_{t+1}$ to gated network consisting of two convolutional layers, followed activation functions, a linear layer and $Sigmoid$ to get pillar description maps $\mathbf{m}_t, \mathbf{m}_{t+1}$, respectively.
\begin{equation}
    \mathbf{m} = \delta(linear(conv(\mathbf{F}))
\end{equation}
where $\delta$ represents $Sigmoid$ to generate pillar description between $0$ and $1$. Then, the results of multiplying description maps with the original feature maps are added to another original feature maps for feature enhancement.
\begin{equation}
    \mathbf{z}_t = \mathbf{F}_t + \mathbf{m}_{t+1} \cdot \mathbf{F}_{t+1}
    \label{equ:z_1}
\end{equation}
\begin{equation}
    \mathbf{z}_{t+1} = \mathbf{F}_{t+1} + \mathbf{m}_t \cdot \mathbf{F}_t
    \label{equ:z_2}
\end{equation}
where $\cdot$ denotes elemental multiplication, and $\mathbf{z}$ represents the modulated feature map. 
% Note that we transform $\mathbf{F}_t$ and $\mathbf{F}_{t+1}$ into the same coordinate before GMF in inference 
GMF is straightforward but adaptively distinguishes between static and dynamic pillars and achieves correct feature fusion. As a result, the feature maps $\mathbf{z} $ contain much more geometric features than $\mathbf{F}$, even if the relevant point is missing. GMF facilitates the extraction of discriminative features of the scene due to feature compensation between multiple frames and is beneficial for pillar association due to the enhanced feature consistency between corresponding pillars. Even without additional supervised signals, the pillar description maps actually embodies the dynamic-static information of the pillars and provides more information for the feature extraction, which is introduced in the ablation experiments.

\subsection{Pillar Association}
After extracting the feature representation of each pillar, we implement pillar association to predict pillar correspondences $\{(P_i^t, P_{i'}^{t+1})\}_{i=1}^{N_p}$ using feature distance. Specifically, the pillar association is in a \textit{query-key} manner where \textit{query} is the feature of $P_i^t$ and \textit{keys} are features of $\{P_j^{t+1}\}_{j=1}^{N_p}$.
% We calculate the feature distance between the query and all keys, and define the corresponding pillar $P_{i'}^{t+1}$ of $P_i^t$ as 
% \begin{equation}
%     \min_{P_j^{t+1}} d_f(\mathbf{z}(P_i^t), \mathbf{z}(P_j^{t+1}))
% \end{equation}
% where $\mathbf{z}(P)$ represents pillar features and $d_f$ denotes the feature distance function, which we define as the inner product operation.
However, the cost of calculating the feature distance between query and all keys is expensive. Therefore, we adopt \textit{Patching} strategy, where the pseudo-image composed of pillars is partitioned into several $s \times s$ patches, named query patches $\{Q^t_i\}_{i=1}^{\frac{N_p}{s^2}}$. For each query patch $Q_i^t$, there exists a corresponding key patch $K_i^{t+1}$ whose patch size is $\alpha s \times \alpha s$ where $\alpha > 1$, 
and the central pillars of the corresponding patches have the same row and column numbers.
The pillars in each query patch only calculate the feature distance with the keys in the corresponding key patch $K_ \cdot ^{t+1}$ and then predict pillar correspondence probability.
We define pillar corresponding probability between $P_i^t$ and $P_j^{t+1}$ as
\begin{equation}
    % pb(i,j) = \max(0, d_f(\mathbf{z}(P_i^t), \mathbf{z}(P_j^{t+1})) )
    pb(i,j) = \frac{exp(\mathbf{z}(P_i^t) * \mathbf{z}(P_j^{t+1}))}{\sum _{k \in K_ \cdot ^{t+1}} exp(\mathbf{z}(P_i^t) *\mathbf{z}(P_k^{t+1}))}
\end{equation}
where $\mathbf{z}(P)$ represents pillar features, $*$ denotes vector inner product. We identify the one with the maximum correspondence probability with $P_i^t$ as its corresponding pillar $P_{i'}^{t+1}$.
The adoption of asymmetric patch sizes ensures that queries at the border of query patch still have sufficient keys to implement pillar association. 
In summary, We adopt \textit{Patching} to achieve greater efficiency and \textit{Asymmetric Patch} to ensure its accuracy.
After acquiring the pillar correspondences $\{(P_i^t, P_{i'}^{t+1})\}_{i=1}^{N_p}$, we calculate the pillar flow of $P_i^t$ through $\mathbf{c}(P_{i'}^{t+1}) - \mathbf{c}(P_i^t)$ where $\mathbf{c}(P)$ represents the center of pillars in the real-world coordinate system.
% In pillar association pipeline, ContrastMotion associates pillars with feature similarity, We feed a pair of point clouds into the encoder and get a pair of feature maps of the same size as the input, and perform the association proces s where query $q$ is $\sigma(P_i^t)$, keys $k$ are
% $\{\sigma(P_j^{t+1})\}_{j=1}^{N_p}$, and values $v$ are the displacement vectors between $P_{i}^{t}$ and $P_{j}^{t+1}$ in the Cartesian coordinate system. If all pillars in time $t+1$ are used as keys, the computational complexity is $O(n^2)$. Therefore, we restrict the keys to $\{p_j^{t+1}|j \in V(P_i^t)\}$, the neighbours of $P_{i}^{t}$ in time $t+1$.

\subsection{Task-specific Post-processing}
\subsubsection{Scene Flow}
Scene flow is defined as a 3D displacement vector between each surface point rather than each pillar, we directly scatter the flow of pillars to points.

% Scene flow is defined as a 3D displacement vector between each surface point rather than each pillar. Directly scattering the motion of pillars to points inevitably introduces the point correspondence errors due to the fact that pillar is a coarse-grained representation. Therefore we employ an efficient post-processing solution. Firstly, we select a reference point randomly for each pillar and performs point association between corresponding pillars obtained from pillar association based on structural information. Specifically, we identify the corresponding point of the reference by maximizing the structural consistency between pillars, and the structural consistency is measured by Chamfer Loss proposed by PointPWC~\cite{wu2019pointpwc}. The query window of reference point is restricted to the corresponding pillar, and all points within the same pillar share the same motion with the reference point, which makes the post-processing scheme  efficient. In addition, our post-processing doesn't introduce new parameters.

% ContrastMotion is a pillar-based model, which has a faster speed and stable memory footprint compared to the point model. Our ContrastFlow utilizes pillar association to estimate the flow of each pillar, while the scene flow is a point flow estimation task. To estimate each point flow in the pillars, we employ a simple and efficient post-processing solution. Specifically, for one sample point in a pillar, we perform point correlation based on structured information, i.e., the point's relative position with respect to surrounding points. Due to the pillar association, the matching search space of the points is restricted within the pillars, and all the points in the same pillar share the same point flow, which is highly efficient. In addition, post-processing introduces no new parameters.

\subsubsection{Motion Prediction}
Generally, the related works~\cite{wu2020motionnet,PillarMotion} predict future motion with the scene motions from the past by assuming consistent velocities and accelerations. 
% For fair comparisons with related methods, We predict the motion for the next 1.0s by average velocities of two past frames.
ContrastMotion estimates the motions with past frames and converts them into velocities, then predict future motion. 

\subsection{Analysis}
Compared to point cloud registration which estimates the transformation matrix between point cloud pairs, scene motion estimates fine-grained motion and is more complex. From the perspective of training samples, our ContrastMotion looks like addressing registration rather than scene motion. Because we utilize data augmentation to generate a pair of point clouds as training sample, and the data augmentation transformation is applied to all points in the point cloud in order to ensure the integrity of the object surface.
\textit{Does the degradation solution occur during training, where the network infers the transformation matrix and obtains the motion of each pillar directly, making the model much less capable of inferring scene motion?}
The reason why ContrastMotion is working relies on the fact that we use a pillar association process instead of the conventional prediction head. In pillar association, we use a query-key manner and for each key we have no additional positional encoding. The distinction between the different pillars(keys) relies on their geometric contextual information rather than on their real position. In pillar association process, the network is agnostic to pillar motion, which avoids the degenerate solution. Thus, even with the training samples generated from the transformation matrix, our model still achieves good performance in real scenes.

% \begin{table*}[htb]
%     \centering
%         \caption{\textbf{Evaluation results on FT3D $\rightarrow$ KITTI Scene Flow.} $^\dag$: Point downsampling.}
%     \scalebox{0.7}{
%     \begin{tabular}{c|c|c|c|c}
%     \hline
%       Method & EPE3D(m)$\downarrow$ & Acc3DS$\uparrow$ & Acc3DR$\uparrow$ & Outliers3D$\downarrow$ \\
%     \hline
%     % \multirow{5}*{8192} & ICP(rigid) \cite{besl1992method} & 0.5181 & 0.0669 & 0.1667 & 0.8712 \\
%     % ~ & FGR(rigid) \cite{zhou2016fast} & 0.4835 & 0.1331 & 0.2851 & 0.7761 \\
%     % ~ & CPD(non-rigid) \cite{myronenko2010point}& 0.4144 & 0.2058 & 0.4001 & 0.7146 \\
%     % \multirow{5}*{8192} & PointPWC \cite{wu2019pointpwc}& 0.2549 & 0.2379 & 0.4957 & 0.6863 \\
%     % ~ & FlowStep3D \cite{kittenplon2021flowstep3d}& 0.1021 & 0.7080 & 0.8394 & 0.2456 \\
%     % ~ & RobOT \cite{shen2021accurate}& 0.0912 & 0.6043 & 0.7939 & 0.3365 \\
%     % ~ & RigidFlow \cite{li2022rigidflow} & 0.0619 & 0.7237 & 0.8923 & 0.2618 \\
%     % ~ & RCP \cite{gu2022rcp} & 0.0763 & \textbf{0.7856} & 0.8921 & 0.1849 \\
%     % \hline
%      % PointPWC  & 0.3648 & 0.0726 & 0.2974 & 0.8579 \\
%      % PoseFlow  & 0.3256 & 0.1104 & 0.2058 & 0.9778 \\
%      % SLIM$^*$  & 0.0688 & \textbf{0.7695} & 0.9342 & 0.2488 \\
%      % FlowStep3D  & 0.1741 & 0.5821 & 0.7397 & 0.3596 \\
%      % RCP$^\dag$ & 0.0974 & 0.6058 & 0.8021 & 0.3263 \\
%      RigidFlow$^\dag$  & \textbf{0.0619} & 0.7237 & 0.8923 & 0.2618 \\
%      ContrastMotion (ours) & 0.0656 & \textbf{0.7382} & \textbf{0.9417} & \textbf{0.1847}\\
     
%      % ContrastMotion (ours) & \textbf{0.0656} & 0.7382 & \textbf{0.9417} & \textbf{0.1847} \\
%     \hline
%     \end{tabular}
%     }
%     \label{tab:KITTT_RESULTS}
% \end{table*}

\begin{table}[htb]
    \centering
        \caption{\textbf{Evaluation results on FT3D $\rightarrow$ KITTI Scene Flow.} These self-supervised methods are trained only on FT3D and evaluated on KITTI Scene Flow dataset for all points. PointPWC, FlowStep3D and RCP are the point-based methods, while ours and SLIM are pillar-based. $^*$: models trained on KITTI-RL. $^\dag$: reproducing experiments. $^\ddag$: 8192 points downsampling.}
    \scalebox{0.7}{
    \begin{tabular}{c|c|c|c|c}
    \hline
      Method & EPE3D(m)$\downarrow$ & Acc3DS$\uparrow$ & Acc3DR$\uparrow$ & Outliers3D$\downarrow$ \\
    \hline
    % \multirow{5}*{8192} & ICP(rigid) \cite{besl1992method} & 0.5181 & 0.0669 & 0.1667 & 0.8712 \\
    % ~ & FGR(rigid) \cite{zhou2016fast} & 0.4835 & 0.1331 & 0.2851 & 0.7761 \\
    % ~ & CPD(non-rigid) \cite{myronenko2010point}& 0.4144 & 0.2058 & 0.4001 & 0.7146 \\
    % \multirow{5}*{8192} & PointPWC \cite{wu2019pointpwc}& 0.2549 & 0.2379 & 0.4957 & 0.6863 \\
    % ~ & FlowStep3D \cite{kittenplon2021flowstep3d}& 0.1021 & 0.7080 & 0.8394 & 0.2456 \\
    % ~ & RobOT \cite{shen2021accurate}& 0.0912 & 0.6043 & 0.7939 & 0.3365 \\
    % ~ & RigidFlow \cite{li2022rigidflow} & 0.0619 & 0.7237 & 0.8923 & 0.2618 \\
    % ~ & RCP \cite{gu2022rcp} & 0.0763 & \textbf{0.7856} & 0.8921 & 0.1849 \\
    % \hline
     PointPWC  & 0.3648 & 0.0726 & 0.2974 & 0.8579 \\
     PoseFlow  & 0.3256 & 0.1104 & 0.2058 & 0.9778 \\
     SLIM$^*$  & 0.0688 & \textbf{0.7695} & 0.9342 & 0.2488 \\
     FlowStep3D  & 0.1741 & 0.5821 & 0.7397 & 0.3596 \\
     RCP$^\dag$ & 0.0974 & 0.6058 & 0.8021 & 0.3263 \\
     % RigidFlow$^\ddag$ & \textbf{0.0619} & 0.7237 & 0.8923 & 0.2618 \\
     ContrastMotion (ours) & \textbf{0.0656} & 0.7382 & \textbf{0.9417} & \textbf{0.1847} \\
    \hline
    \end{tabular}
    }
    \label{tab:KITTT_RESULTS}
\end{table}

\begin{table}[htb]
    \centering
    \caption{\textbf{Self-supervised training \& evaluation on nuScenes scene flow.} \textit{Zero} predicts that the environment is static.}
    \label{tab:nuScene_flow}
    \scalebox{0.8}{
    \begin{tabular}{c|c|c|c}
        \hline
         \multirow{2}*{Method} & \multicolumn{2}{|c|}{Moving} & Stat. \\ 
         ~ & EPE3D(m)$\downarrow$ & Acc3DR$\uparrow$ & EPE3D(m)$\downarrow$ \\ \hline
         Zero & 0.6381 & 0.1632 & 0.5248 \\
         PointPWC & 0.3539 & 0.2543 & 0.1974 \\
         PoseFlow & 0.7399 & 0.0000 & 0.0570 \\
         SLIM & 0.1050 & \textbf{0.7365} & 0.0925 \\
         ContrastMotion(ours) & \textbf{0.0925} & 0.7082 & \textbf{0.0545} \\ \hline
    \end{tabular}
    }
\end{table}

% 
\begin{table*}[htb]
    \centering
        \caption{\textbf{Comparison with the state-of-the-art results on the nuScenes motion prediction}. We report the mean and median errors on the three speed groups. \textit{Self} indicates self-supervised methods trained with nuScenes, and \textit{Pre.} indicates the methods that are not trained with the annotations of nuScenes but are supervised pre-trained on two scene flow datasets. \textit{Zero} predicts that the environment is static.}
    \scalebox{0.9}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}*{Method} & \multirow{2}*{Sup.} & \multicolumn{2}{|c|}{Static} & \multicolumn{2}{|c|}{Speed $\le$ 5m/s} & \multicolumn{2}{|c}{Speed $\ge$ 5m/s} \\
    ~ & ~ & Mean & Median & Mean & Median & Mean & Median \\
    \hline
    % Static Model & - & \textbf{0.0000} & \textbf{0.0000} & 0.6111 & 0.0971 & 8.6517 & 8.1412 \\
    Zero & - & \textbf{0.0000} & \textbf{0.0000} & 0.6111 & 0.0971 & 8.6517 & 8.1412 \\
    % FlowNet3D & Full & 0.0410 & 0.0000 & 0.8183 & 0.1782 & 8.5261 & 8.0230 \\
    % HPLFlowNet & Full & 0.0041 & 0.0002 & 0.4458 & 0.0969 & 4.3206 & 2.4881 \\
    FlowNet3D \cite{liu2019flownet3d} & Pre. & 2.0514 & \textbf{0.0000} & 2.2058 & 0.3172 & 9.1923 & 8.4923 \\
    HPLFlowNet \cite{gu2019hplflownet} \ & Pre. & 2.2165 & 1.4925 & 1.5477 & 1.1269 & 5.9841 & 4.8553 \\
    PillarMotion \cite{PillarMotion} & Self & 0.1620 & 0.0010 & 0.6972 & 0.1758 & 3.5504 & 2.0844 \\
    ContrastMotion (ours) & Self & 0.0829 & \textbf{0.0000} & \textbf{0.4522} & \textbf{0.0959} & \textbf{3.5266 }& \textbf{1.3233} \\
    \hline
    \end{tabular}
    }
    \label{tab:NUSCENES_RESULTS}
\end{table*}

\begin{table*}[htb]
    \centering
        \caption{\textbf{Ablation study for different modules of ContrastMotion.} We evaluate each model on nuScenes motion prediction and report mean errors. Ground Mask: Removing estimated ground points before feeding to network. Gated Block: \textit{Gated Multi-frame Fusion Block}.}
    \scalebox{0.9}{
    \begin{tabular}{c|c c|c|c|c|c|c}
    \hline
        Method & SD--Loss & PointInfoNCE Loss & Ground Mask & GMF & Static & Speed $\le$ 5m/s & Speed $>$ 5m/s\\
        \hline
         % (newcomer) & & \checkmark & & & 0.1396 & 0.9147 & 4.2056 \\
         (a) & \checkmark & & & & 0.1377 & 0.7791 & 3.9497 \\
         (b) & \checkmark & & & \checkmark & \textbf{0.0682} & 0.4579 & 3.9872 \\
         (c) & \checkmark & & \checkmark & \checkmark & 0.0829 & \textbf{0.4522} & \textbf{3.5266} \\
         (d) & & \checkmark & \checkmark & \checkmark & 0.0837 & 0.6546 & 3.9601 \\
    \hline
    \end{tabular}
    }
    \label{tab:ABL}
\end{table*}




==> sections/related.tex <==
\subsection{Supervised Motion Learning}
This task aims to estimate motions and predict the future locations of various agents via past information~\cite{PillarMotion}. The previous works~\cite{ma2019trafficpredict,sadeghian2019sophie} formulate this task as a trajectory problem based on 3D object detection and tracking. 
% Such a paradigm relies on accurate detection and cannot avoid the destruction of unknown object classes. 
Another active research line~\cite{wu2020motionnet,lee2020pillarflow,wei2021pv,li2022sctn,wang2022sti} estimate the motions in a end-to-end framework. 
% For instance, MotionNet~\cite{wu2020motionnet} leverages the spatio-temporal pyramid network to perform joint motion prediction and perception with the extracted spatial and temporal features. 
However, 3D labeling on large-scale point clouds requires complex processes and labor-intensive human efforts, and there are significant discrepancies between cross-scenes and cross LiDAR captured data. 
% As a result, researchers tend to explore motion estimation in unsupervised learning.

% Moreover, Scene flow which involves consecutive frames to estimate 3D displacement vectors is the another research line for scene motion learning. However, current methods~\cite{li2021self, hur2021self, kittenplon2021flowstep3d, wu2019pointpwc} process the significantly sub-sampled point clouds in the training and inference pipelines due to the heavy cost of memory and computation on raw data. Moreover, these approaches trained with synthetic data show the limited performance in the real scenes. As a result, researchers tend to explore the motion estimation in BEV and pillar representation. MotionNet~\cite{wu2020motionnet} extracts spatial and temporal features with the spatio-temporal pyramid network to perform joint motion prediction and perception in a BEV map. PillarFlow~\cite{lee2020pillarflow} achieves 2D BEV flow estimation with a coarse-to-fine paradigm adapted from PWC-Net~\cite{sun2018pwc}. 

% Some approaches~\cite{wu2020motionnet} formulate this task as a trajectory problem, which predicts the future positions of various agents from past observations. Among them, the multi-stage models () rely on the detection and track pipeline, which is more likely to accumulate errors and unable to track unknown classes of agents, and the end-to-end methods () leverage contextual knowledge of the scene and generalize to estimate the motion of agents correctly. Another active research line (Behl et al. 2019; Liu, Qi and Guibas 2019; Wang et al. 2020; Lee et al. 2020; Mittal, Okorn and Held 2020; Jund et al. 2021) involves two consecutive point clouds and estimates 3D vectors of each point or voxel from the source point cloud to the corresponding location in the target point cloud. MotionNet (Wu, Chen and Metaxas 2020) represents the raw point clouds into BEV maps, and outputs both perception and motion information based on a Spatio-temporal pyramid network. PillarFlow (), PointPWC (PointPWC) utilize the coarse-to-fine Network adapted from PWC-Net (PWC-Net) for scene flow estimation. Although slightly different, recent supervised learning methods estimate scene flow by understanding point cloud scenes. However, dense ground truth flow labels in real data are challenging to acquire. These methods trained with synthetic data exhibit limited performance due to the domain gap. Moreover, there are many corresponding points in the synthesized data or processed data, but in the real scene, the correspondence of points cannot be guaranteed due to the ego-motion and movement of agents (pillar motion).
\subsection{Self Supervised Motion Learning}
% In contrast to supervised learning, unsupervised learning opens up the possibility to utilize a practically infinite train data size and has grown significantly with the explosive growth of low-cost data. 
% In various domains, unsupervised pre-trained methods~\cite{devlin2018bert,he2022masked,xie2020pointcontrast} exploring effective representations achieve promising results. 
In the field of the point cloud, There are already self-supervised \cite{wu2019pointpwc,mittal2020just,kittenplon2021flowstep3d,li2021self,hur2021self,kittenplon2021flowstep3d,wu2019pointpwc} and non-learning~\cite{li2021neural} methods for motion estimation. PointPWC~\cite{wu2019pointpwc} estimates the motions with a coarse-to-fine paradigm and introduces the losses for scene consistency, smoothness and shape approximation. However, these methods perform significant sampling in the training and inference pipelines due to the heavy costs of memory and computation. Instead of dense motion, researchers tend to explore the motion in pillar representation. PillarMotion~\cite{PillarMotion} introduces structural consistency augmented with motion masking and a cross-sensor (LiDAR and camera) regularization to predict the motion of pillars. SLIM~\cite{baur2021slim} proposes a self-supervised model for motion estimation and segmentation in a BEV map. However, these methods are similar to previous scene flow methods by mainly using the point-level structure consistency and regularization between consecutive frames, which suffer from the dynamic changes of scenes. 
% Therefore, We propose a self-supervised motion estimator based on feature consistency to reduce the effect of data-level correspondences.

% Further, using unsupervised learning approaches solve downstream tasks directly is rapidly growing. From zero labels, MODEST \cite{you2022learning} leverages the common scene properties to define ephemeral (mobile) objects as the seed labels and bootstraps an improvement mobile object detection by self-training. In the field of point cloud motion, PointPWC~\cite{wu2019pointpwc} introduces the Chamfer Loss, smoothness constraint and Laplacian regularization for scene consistency, local spatial smoothness, and shape characteristics approximate respectively. \cite{mittal2020just} introduce the Nearest Neighbor Loss to penalize the error between the predicted point cloud and the target point cloud, and the work also proposes the Cycle Consistency Loss that comes from reconstructing the original point cloud from the predicted point cloud to avoid degenerate solutions. FlowStep3D~\cite{kittenplon2021flowstep3d}, a recurrent architecture method, learns an unrolled iterative alignment procedure to refine motion estimation. PillarMotion~\cite{PillarMotion} involves structural consistency augmented with motion masking and a cross-sensor (lidar and camera) regularization to predict the motion of the scene. 


\subsection{Contrastive Learning}
Contrastive learning~\cite{radford2021learning,bai2022point} has been widely used due to the great potential in pre-training and feature correspondence learning. 
% For instance, CLIP~\cite{radford2021learning} bridges the text and image domains with contrastive learning, which can be used not only for text and image matching problems but for zero-point prediction. 
In the point cloud field, PointContrast~\cite{xie2020pointcontrast} proposes a pre-trained method for learning representations via matching corresponding points in different views. Specifically, it establishes the connections of corresponding points in different perspectives with the proposed PointInfoNCE to enhance the representation of the model. However, The pretext task only involves point-level correspondence matching which completely ignores the spatial configuration and context in the scene \cite{hou2021exploring}, leading to a limited performance in motion tasks.
